An Analytic Approximation to the Bayesian Detection Statistic for Continuous Gravitational Waves

We consider the Bayesian detection statistic for a targeted search for continuous gravitational waves, known as the $\mathcal{B}$-statistic. This is a Bayes factor between signal and noise hypotheses, produced by marginalizing over the four amplitude parameters of the signal. We show that by Taylor-expanding to first order in certain averaged combinations of antenna patterns (elements of the parameter space metric), the marginalization integral can be performed analytically, producing a closed-form approximation in terms of confluent hypergeometric functions. We demonstrate using Monte Carlo simulations that this approximation is as powerful as the full $\mathcal{B}$-statistic, and outperforms the traditional maximum-likelihood $\mathcal{F}$-statistic, for several observing scenarios which involve an average over sidereal times. We also show that the approximation does not perform well for a near-instantaneous observation, so the approximation is suited to long-time continuous wave observations rather than transient modelled signals such as compact binary inspiral.

==> Metric_dat.tex <==
\newcommand{\PKA}{0.154}
\newcommand{\PKB}{0.234}
\newcommand{\PKC}{-0.0104}
\newcommand{\PKI}{0.388}
\newcommand{\PKK}{-0.0207}
\newcommand{\PKL}{-0.0805}
\newcommand{\PKKI}{-0.0533}
\newcommand{\PKLI}{-0.207}
\newcommand{\OiA}{0.167}
\newcommand{\OiB}{0.206}
\newcommand{\OiC}{-0.0060}
\newcommand{\OiI}{0.373}
\newcommand{\OiK}{-0.0120}
\newcommand{\OiL}{-0.0385}
\newcommand{\OiKI}{-0.0321}
\newcommand{\OiLI}{-0.103}
\newcommand{\oA}{0.666}
\newcommand{\oB}{0.013}
\newcommand{\oC}{0.0802}
\newcommand{\oI}{0.679}
\newcommand{\oK}{0.1604}
\newcommand{\oL}{0.6527}
\newcommand{\oKI}{0.236}
\newcommand{\oLI}{0.961}
\newcommand{\HiA}{0.078}
\newcommand{\HiB}{0.226}
\newcommand{\HiC}{0.0000}
\newcommand{\HiI}{0.305}
\newcommand{\HiK}{0.0000}
\newcommand{\HiL}{-0.1479}
\newcommand{\HiKI}{0.0000}
\newcommand{\HiLI}{-0.485}


==> tag.tex <==
\def\commitID{commitID: 71d775b4edda5b4e24cf000473d29b42b04a11d7}
\def\commitDATE{ Sat Aug 4 21:20:29 2018 -0400}
\def\commitIDshort{commitID: 71d775b}
\def\commitSTATUS{CLEAN}

